Hide to See: Reasoning-prefix Masking for Visual-anchored Thinking in VLM Distillation

Recent think-answer approaches in VLMs, such as Qwen3-VL-Thinking, boost reasoning performance by leveraging intermediate thinking steps before the final answer, but their computational cost becomes substantial, especially for larger VLMs. To distill such capabilities into compact think-answer VLMs, a primary objective is to improve the student's ability to utilize visual evidence throughout its reasoning trace, as long think-answer traces suffer from visual forgetting issues. To this end, we introduce a novel think-answer distillation framework that encourages the student to anchor its thinking on visual information by masking the student's salient reasoning prefixes. To compensate for such masked textual cues, the student is encouraged to rely more on visual evidence as an alternative source of information during distillation. Our masking strategies include: 1) token-wise salient reasoning-prefix masking, which masks high-influence reasoning prefixes selectively for each next-token prediction, and 2) self-paced masking budget scheduling, which gradually increases the masking scale according to distillation difficulty, measured by the discrepancy between teacher--student distributions. In the distillation phase, the student is guided by our salient reasoning-prefix mask, which blocks both future tokens and salient reasoning cues, in place of the standard causal mask used for auto-regressive language modeling. Experimental results show that our approach outperforms recent open-source VLMs, VLM distillation, and self-distillation methods on multimodal reasoning benchmarks, while further analyzes confirm enhanced visual utilization along the student thinking process.

==> tab/entropy.tex <==
\begin{table}[]
    \centering
        \renewcommand{\arraystretch}{1.15}
    \begin{tabular}{l|cc||c|c}
    \hline
         &  Pass@1 & Pass@8 & Entropy & Avg. Length\\ \hline
    Base {\small{\textit{Qwen3-VL-2B-Thinking}}} & 24.12 & 26.99 & 0.70 & 1471\\ \cdashline{1-5}[0.2pt/1pt]
    Na\"ive Response Distillation     & 38.26 & 39.88 & 0.34 & 803 \\ 
    Masking-KD (ours) & 47.34 & 47.60 & 0.22 & 346 \\
    \hline
    \end{tabular}
    \vspace{0.2cm}
    \caption{Caption}
    \label{tab:placeholder}
\end{table}
